SHARCS: Efficient Transformers through Routing with Dynamic Width Sub-networks

We introduce SHARCS for adaptive inference that takes into account the hardness of input samples. SHARCS can train a router on any transformer network, enabling the model to direct different samples to sub-networks with varying widths. Our experiments demonstrate that: (1) SHARCS outperforms or complements existing per-sample adaptive inference methods across various classification tasks in terms of accuracy vs. FLOPs; (2) SHARCS generalizes across different architectures and can be even applied to compressed and efficient transformer encoders to further improve their efficiency; (3) SHARCS can provide a 2 times inference speed up at an insignificant drop in accuracy.

==> emnlp2023-latex/sections/02_related_work.tex <==
\paragraph{Efficient non-adaptive inference} In the context of non-adaptive methods, numerous studies in the literature have improved the inference efficiency of transformers through various techniques such as knowledge distillation \cite{knowledge_distillation} into smaller models \cite{distilbert,mobile_bert,dynabert,tinybert}, pruning unimportant weights of the model \cite{cofi,block_pruning,movement_pruning,metapruning}, and weight quantization \cite{qbert,ibert} to store weights of a network with lower precision values. The aforementioned approaches result in smaller and more efficient albeit fixed and static models. 
%As a consequence, it remains unclear whether the resulting efficient networks are excessively complex for simpler samples or overly simplified for more challenging ones. Moreover, adjusting the computational complexity of the model based on each use-case can be time-consuming and costly \cite{deebert}; obtaining a network suited to a different use case typically involves obtaining a new model with a different architecture based on specific constraints \cite{block_pruning,cofi,movement_pruning} or undertaking expensive knowledge distillation techniques using general-purpose \cite{distilbert} or augmented corpora \cite{dynabert}, or a combination of both \cite{tinybert}. These complexities highlight the need for alternative approaches that can address these challenges in a more cost-effective manner. 
% \paragraph{Efficient Adaptive inference.} Another line of work have proposed adaptive inference methods that allow the network to allocate varying amounts of compute for each sample. The predominant technique in this area is early exiting via adding internal classifiers to intermediate layers \cite{RTJ,shallow_deep,deebert,branchynet,pabee,fastbert}: 
% %The internal classifiers implicitly learn to identify simpler samples and early exit the computation so the model does not waste extra compute on them. Early exiting methods use different measures to determine when to exit the computation: 
% To early exit, prior work either use the confidence score of internal classifiers' predictions \cite{RTJ,deebert}; or the entropy of these predictions \cite{fastbert}; or a module that predicts whether a layer should early exit or not\cite{berxit}; or a patience based change in these internal prediction \cite{pabee}; or a hash based mechanism to do token level early exiting \cite{hashee}.
% \cite{RTJ} early exits if the confidence score of an internal classifier is higher than a threshold; \cite{deebert} uses a similar early exiting approach and trains the network with the main classifier and internal classifier in two stages; \cite{fastbert} trains internal classifier with knowledge distillation \cite{knowledge_distillation} from the last layer's classifier; \cite{hashee} uses a non-learnable hash-based mechanism to do early exiting per token instead of the sequence; \cite{berxit} takes a slightly different approach and uses a binary light-weight classifier that determines whether any internal classifier should exit or not; 

%In a separate but related line of work \cite{moe,moe_expert_choice} introduce mixture of expert architecture (MOE) which uses routing to different feed forward networks inside the transformer block to scale number of parameters while keeping the inference flops the same. However, It is important to note that MOE is not a general purpose approach that can make any network's inference adaptive and efficient.


% Pruning methods \cite{cofi,movement_pruning,block_pruning,switch_transformer,metapruning} improve efficiency by removing parameters that contribute less to the network's accuracy on a task. Distilling the knowledge of a network into a smaller student network \cite{distilbert, tinybert, minilm, mobile_bert,dynabert} is another common approach in making inference more efficient. Another line of work use quantization \cite{qbert,ibert} to compress weights of a network into low-precision values. 


% Our approach is different in two ways compared with the existing adaptive approaches. We use a router and propose a novel approach that leverages training historyto train the router. 

==> emnlp2023-latex/sections/03_method.tex <==
% \begin{figure*}[ht!]
%   % \begin{minipage}
%   %   \raggedright
%   %   \begin{subfigure}[]
%   %     \centering
%   %     \includegraphics{emnlp2023-latex/figures/detail_arch.pdf}
%   %     \caption{Reducing Fully-connected projection layer width}
%   %     \label{fig:subfig1}
%   %   \end{subfigure}
%   %   \begin{subfigure}
%   %     \centering
%   %     \includegraphics[width=0.69\textwidth}]{emnlp2023-latex/figures/train_router.pdf}
%   %     \caption{Reducing MHA projection layer (key, query, or value) width}
%   %     \label{fig:subfig3}
%   %   \end{subfigure}
%   %   % \begin{subfigure}{0.3\linewidth}
%   %   %   \centering
%   %   %   \includegraphics[width=\linewidth]{emnlp2023-latex/figures/adaptive_router.pdf}
%   %   %   \caption{Adaptive width with routing}
%   %   %   \label{fig:subfig3}
%   %   % \end{subfigure}
%   % \end{minipage}
%   \caption{Reducing the width of different components in transformer networks.
%   \label{fig:dim_reduction}
% \end{figure*}

% \begin{figure*}[ht!]
%     \includegraphics[width=\textwidth]{emnlp2023-latex/figures/all.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure*}


% We aim to improve the efficiency of any network's inference by enabling it with a means to allocate varying amounts of compute for different input samples. To achieve this, we propose to incorporate a lightweight router network that determines with which capacity the network should process each input. To train the router, we introduce a novel approach that leverages the network's confidence scores for different samples during training (section \ref{section_train}).

%Given \textit{any} transformer network with $L$ layers, our goal is to learn a set of sub-networks within the network (including the network itself), and process an input sample with one of the sub-networks that is appropriate based on the sample hardness. These sub-networks have the same number of layers but vary only in their layer widths.
 %  %a set of sub-networks within the network (including the network itself), and process an input sample with one of the sub-networks that is appropriate based on the sample hardness. These sub-networks have the same number of layers but vary only in their layer widths.
%This will enable us to deploy each sub-network to a suitable device based on its resource constraints.
% Toward this,  we propose a novel approach to train a light-weight router (Section \ref{subsub_router}) on top of any network %while training the network,
% . 
% We create the labels for training the router based on the confidence scores of the sub-networks. 
%adaptively choose a sub-network according to the the input sample's compelxity.
%to process each input sequence based on its complexity. These sub-networks have the same number of layers and only differ in the width of their layers (Section \ref{subsub_adaptive_sub_network}). We train the router with the labels generated dynamically over the training based on the confidence scores of the predictions of the sub-networks (Section \ref{section_router_objective}). During inference, the router selects one sub-network to process the sample, which produces the final classification prediction. (Section \ref{section_inference}). 
%An overview of the architecture of our adaptive width network is illustrated in Figure 2. 
  
% 1. \textbf{Non-adaptive module} which consists of the first $K$ transformer layers of the original model. By adjusting the value of $K$ we can the balance accuracy and the computational cost for different devices. 
% We leave the first $K$ layers (aka non-adaptive module) of the model intact, where $K$ is a hyperparameter. %This module computes a contextualized representation of the input which will be used as the input to the router and the deeper layers of the model. 
% The non-adaptive module is identical to the corresponding part in the original network, therefore we do not discuss it further in the paper.
%\textbf{Router} which.
% The router (section \ref{sub_router}) is a lightweight fully-connected classifier that takes the hidden states of the non-adaptive module as input. It then determines a reduction factor to be applied to the adaptive module, which in turn determines the width of various components during the forward pass (section \ref{sub_adaptive_component}).
%3. \textbf{Adaptive width module} which consists of the last $L\!-\!K$ layers of the original network that has been made adaptive via training its sub-networks. Only one of the sub-networks within the adaptive module processes the input and get the final hidden representations. These representations will be passed to a linear classifier to get the final predictions of the task. 

% We first describe the adaptive module and will next discuss how our router selects sub-network.

% \subsubsection{Router}
% \label{subsub_router}
% The goal of the router module is to learn select a sub-network with an appropriate width to process each input sequence. As Figure \ref{fig:architecture} illustrates, the router is a simple fully-connected classifier with one hidden layer and a $ReLU$ non-linearity. This module gets the intermediate representations $h$ of the non-adaptive module as the input and selects the appropriate reduction factor from $\{r_i\}_{i=1}^M$ to be applied on adaptive-module.

% \subsection{Router}

% \subsection{Adaptive-width component}
% \label{sub_adaptive_component}
% %The adaptive module consists of $M$ sub-networks $\{N_1, N_2, ..., N_M\}$ which share their parameters with the original network. The ratio of the width of each component in $N_i$ to the width of the corresponding component in the original network is $r_i$ where $0 \leq r_i \leq 1$. Later in this section, we will describe how we define the width of different components within a layer.\\
% % Based on the reduction factor $r$ selected by the router, the adaptive module will run each component with $r$ times smaller width. Later in this section, we will define the width of different components within a transformer layer.

% % Given an input sequence $x$, after computing the intermediate representation $h \in \mathbb{R}^{l \times D_{model}}$ by the non-adaptive module, one of the sub-networks such as $N_j$ will be selected by the router to further process $h$.
% Given an input sequence $x$, after computing the intermediate representation $h \in \mathbb{R}^{l \times D_{model}}$ by the non-adaptive module, and the reduction factor $r$ by the router, the adaptive module takes $h$ as input and runs with $r$ times smaller width. Before passing $h$, we reduce its dimension by only selecting the first $D_{model} \times r$ dimensions. For instance, if $D_{model}=768$ and $r=0.25$, the input to the adaptive module will be 192 dimensional. In this paper, whenever we decrease a dimension of a component from $D$ to $D^\prime$, it exclusively uses the first $D'$ dimensions and disregards the remainder in the computations. 



% In what follows we describe how we reduce the width of different components 
% %in a sub-network with 
% by a reduction factor $r$ which is also depicted in Fig. \ref{fig:dim_reduction}. 
% %We also assume that the dimension of the input to the network $N_i$ is reduced by a factor of $r_i$. Throughout the paper, whenever the width of a component is reduced from $D$ to $D^\prime$, the first $D^\prime$ dimensions of that component is selected and will be fed to the deeper layers. For instance, if the original input is 768 dimensional and $r_1=0.25$, the input to the first network is the first 192 dimensions. In what follows, we describe how we reduce the widths of different components of a transformer layer. 
% \paragraph{Reducing MHA width.} We reduce the width of MHA %in network $N_j$ 
% %by a factor of $r_j$ 
% using the following steps:

% 1. The input dimension $D_{model}$ of self-attention projection matrices $W_K$, $W_Q$, $W_v$ is decreased by a factor of $r$. We do not change the output dimension $D_{head}$ of the linear projections.

% 2.%Sub-network $N_j$ 
%  The adaptive module only computes the output of the first $H \times r$ heads and disregards the other heads. Therefore the dimensionality of $O_{heads}$ is decreased to $D_{model} \times r$.

% 3. For the output projection $W_o$ of MHA, the input and output dimensions, which are both equal to $D_{model}$, are reduced by a factor of $r$. Therefore the output of MHA will have a dimensionality of $D_{model} \times r$.

% Throughout all the changes above, we do not alter the sequence length of the input or any of the hidden states. 
% % It is worth mentioning that as the input and output dimensions of all the projection layers have been reduced by a factor of $r_j$, the total flops of the projections will be reduced by a factor of $r_j^2$.
% \paragraph{Reducing FFN width.} Similar to the output projection $W_o$ of MHA, the input and output dimensions of the feed-forward layers $W1$ and $W2$ in the FFN are reduced by a factor of $r$. Therefore, the output dimension of all the adaptive layers%in network $N_i$ 
%   are reduced by a factor of $r$ to $D_{model} \times r$.

% It is important to note that majority of operations in FFN and MHA components are comprised of matrix multiplications and reducing the input and output dimensions of these multiplications by a factor of $r_j$ will reduce their flops by a factor of $r_j^2$.
% \paragraph{Reducing layernorm width.} We also reduce the width of the layer norm parameters by a factor of $r$. In our experiments, we find it beneficial to initialize the layernorm parameters with the corresponding first dimensions of original layernorm parameters instead of training them from scratch.
% % As the width of both the input and outputs of MLP and MHA have been reduced, the width of the layernorms should also be reduced to the same size. To do that, we create an individual layernorm with the required width for each of the sub-networks, both at the output of MLP and MHA.
% \paragraph{Reducing pooler width.} In line with the literature on using transformer encoders for classification, we add a pooler layer $W_{pooler}$ before the linear classifier which operates on the [CLS] token. The linear classifier will then gets this output as input and produces the logits of the classes. We reduce the input dimension of $W_{pooler}$ to $D_{model} \times r$ and keep the output dimension $D_{model}$. Note that the same output dimensionality allows us to train a single classifier for all the sub-networks.



% In contrast to previous work which just reduce the number of heads and the intermediate layer of MLP in the transformer layer, we make the network further efficient by reducing the size of the input. This will result in 16 times less computation for the projection layers in Multi-head attention and each layer in the MLP. To reduce the dimension of the input, we slice out the last $N - d$ dimensions of the hidden representation and just keep the first $d$ values. Similar to ..., we privatize layer-norms for all the adaptive width layers and initialize each one from the first dimensions of the corresponding full width layer-norms in the original network.

% \subsubsection{Router}
% \label{subsub_router}
% The goal of the router module is to learn select a sub-network with an appropriate width to process each input sequence. As Figure \ref{fig:architecture} illustrates, the router is a simple fully-connected classifier with one hidden layer and a $ReLU$ non-linearity. This module gets the intermediate representations $h$ of the non-adaptive module as the input and selects the appropriate reduction factor from $\{r_i\}_{i=1}^M$ to be applied on adaptive-module.


